Conditional Nested Pattern Matching in Interaction Net

Interaction nets are a form of restricted graph rewrite system that can serve as a graphical or textual programming language. As such, benefits include one-step confluence, ease of parallelism and explicit garbage collection. However, some of these restrictions burden the programmer, so they have been extended in several ways, notably to include data types and conditional rules. This paper introduces a further extension to allow nested pattern matching and to do so in a way that preserves these benefits and fundamental properties of interaction nets. We also show that by introducing a translation to non-nested matching, this extension is conservative in rewriting. In addition, we propose a new notation to express this pattern matching.

==> eptcsdata.tex <==
\providecommand{\firstpage}{90}
\providecommand{\publicationstatus}{S. Alves and I. Mackie (Eds.): 13th International Workshop\\
on Developments in Computational Models 2023 (DCM'23).\\
EPTCS 408, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.408.6}{10.4204/EPTCS.408.6}}
\pdfoutput=1

